Intermittency for the stochastic heat and wave equations with generalized fractional noise

We are looking at the stochastic heat and wave equations with different types of fractional noise. We are interested in the intermittency property and Lyapunov exponent for the solution. First we look at the equation driven by the Dobric-Ojeda noise and we show that the Lyapunov exponent matches that of the equation driven by standard fractional noise as obtained by Hu, Huang, Nualart, Tindel (2015) and Balan, Conus (2016). In the second part, we introduce a generalized fractional noise that includes both standard fractional noise and Dobric-Ojeda noise. It shows that, in this specific situation, the correlation structure of the noise does not change the Lyapunov exponent. We conjecture that this result would hold more generally

==> chapter1old.tex <==
%% This is an example first chapter.  You should put chapter/appendix that you
%% write into a separate file, and add a line \include{yourfilename} to
%% main.tex, where `yourfilename.tex' is the name of the chapter/appendix
%% file. You can process specific files by typing their names in at the
%% \files= prompt when you run the file main.tex through LaTeX.  

\chapter{Introduction}
\section{Problem Setup}
We consider the stochastic heat equation (SHE)\\
\begin{align}
\left\{
\begin{array}{l}
\displaystyle
\label{eqn:DO process}
    \frac{\partial}{\partial t} u(t,x)=\frac{1}{2}\Delta u(t,x)+ u(t,x)\dot{W},\\\rule{0ex}{1.5em}
    u(0,x)=u_0,
    \end{array}
\right.
\end{align}
also known as the Parabolic Anderson model, and the stochastic wave equation (SWE)\\
\begin{align}
\label{eqnwave:DO process}
\left\{
\begin{array}{l}
\displaystyle
    \frac{\partial^2}{\partial t^2} u(t,x)=\Delta u(t,x)+  u(t,x)\dot{W},\\\rule{0ex}{1.5em}
    u(0,x)=u_0,\\
    \frac{\partial}{\partial t}u(0,x)=v_0,
    \end{array}
\right.
\end{align}



where $t>0, x\in \mathbb{R}^d$, $\Delta$ stands for the Laplacian operator on $\mathbb{R}^d$, $u_0$ and $v_0$ are universal constants. We are interested in two cases for $\dot{W}$ in this study. (i) Dobri\'{c}-Ojeda noise defined in Definition \ref{DO noise def}. (ii) the generalized fractional noise (an interpolation of standard fractional noise and Dobri\'c-Ojeda noise), which will be introduced in Chapter 5. 



\begin{definition}[Dobri\'{c}-Ojeda noise]
\label{DO noise def}
Let $H\in (0,1)$. Let $F$ be a function such that 
\begin{align}
\label{eqn: variance}
    \int_0^t\int_0^L F^2(y,s)s^{2H-1}dyds<\infty.
\end{align}
This condition ensures that $F $ is W-integrable.

We define
\begin{align}
\label{Do definition eqn}
&\int_0^t\int_0^LF(y,s)W(dyds):=\int_0^t\int_0^LF(y,s)s^{H-1/2}W_0(dyds).
\end{align}
where $W_0$ stands for the time white noise with space covariance function $f$. \\
Informally, $W_0$ is defined as following:
\begin{align*}
    E[\dot{W}_0(s,x)\dot{W}_0(t,y)]=\delta_0(t-s)f(x-y),
\end{align*}
where $\delta_0$ is the delta function.

By \eqref{eqn: variance}, the integral \eqref{Do definition eqn} on the right is well defined by Walsh\cite{walsh1986} and Dalang\cite{Dalang1999}.\\
For Dobri\'c-Ojeda noise, we have informally
\begin{align*}
        E[\dot{W}(s,x)\dot{W}(t,y)]=s^{H-1/2}t^{H-1/2}\delta_0(t-s)f(x-y).
\end{align*}
In other words, this corresponds to 
\begin{align}
    W(dsdy)=s^{H-1/2}W_0(dsdy).
\end{align}

\end{definition}


There exists other definition for Dobri\'{c}-Ojeda noise. Here we assume the process has no drift. The Dobri\'c-Ojeda noise (in short, we will call it DO noise for convenience) is widely used in finance applications, see Wildman~\cite{Mackenzie2016}, Wildman and Conus~\cite{wildmanConus}, Carr and Itkin~\cite{carritkin}
The most useful property of the DO process is that it is a semi-martingale, and can be represented as an Ito diffusion.\\
Noted that DO noise applications in finance usually only involves time, e.g., 
\begin{align}
    W(ds)=s^{H-1/2}W_0(ds).
\end{align}



We also find that the model using the Dobri\'c-Ojeda process does, in fact, approximate the option price given using fractional Brownian motion when the parameter $H$ is similar, which motivates us to generalize the fractional noise for applications in stochastic PDEs.

Here we give a brief introduction to fractional Brownian motion. It was introduced by Mandelbrot and Van Ness~\cite{mandelbrot1968}, as a Gaussian process with time dependence through the parameter $H$, called Hurst index, which estimates the intensity of long-range dependence.

\begin{definition}[Fractional Brownian motion]
Let $H\in (0,1)$. Fractional Brownian motion with Hurst index $H$ is a real-valued Gaussian process $(Z_H(t))_{t\in [0,\infty)}$, where Hurst index, $H\in (0,1)$, such that $Z_H(0)=0$ almost surely and \\
\begin{align}
    E[Z_H(t)Z_H(s)]=\frac{1}{2}\{t^{2H}+s^{2H}-|t-s|^{2H}\},
\end{align}
for all $t,s\geq 0$.
\end{definition}

For values of $H >\frac{1}{2}$, the increments of the process are positively correlated and the closer $H$ is to 1, the stronger long-memory the process exhibits. Conversely, if $H < \frac{1}{2}$ , the increments of fractional Brownian motion are negatively correlated. Notice that for DO process no matter what $H$ we choose, it will always have independent increments. The parameter $H$ does not have the same meaning in the correlation sense.

Fractional Brownian motion is widely used in financial applications as well, but in most cases, it's only the SDE(without space term). For example, the modifications of Black-Scholes SDE by Hu and \O skendal~\cite{huoksendal2003}
\begin{align}
    dS_t=S_t (\mu dt+\sigma dZ_H(t)),
\end{align}
with the solution given by:
\begin{align}
S_t=S_0 \exp\{\sigma Z_H(t)+\mu t-\frac{1}{2}\sigma^2 t^{2H}\}.   
\end{align}
In Wildman's thesis \cite{Mackenzie2016}, it shows that the Hurst index of S\&P 500 index is approximately 0.61 with a 95\% confidence interval (0.57,0.69). But since all the theory of stochastic integration for fractional Brownian motion is in Wick sense, we can not directly use any martingale property.

In the context of SPDEs, the fractional noise with covariance function is informally defined by
\begin{align}
    E[ W(t,x) W(s,y)]=\frac{1}{2}\{t^{2H}+s^{2H}-|t-s|^{2H}\}f(x-y).
\end{align}
 Then if we take the derivative with respect to $t$ and $s$, we have
 \begin{align}
     E[\dot W(t,x)\dot W(s,y)]= \alpha_H |t-s|^{2H-2} f(x-y),
 \end{align}
where $\alpha_H=H(2H-1)$. This is a known result in \cite{Balan2016}.



\begin{remark}
If we take $H=1/2$, then $\dot{W}$ becomes the space-time white noise, and $Z_H(t)$ becomes standard Brownian motion.
\end{remark}

\section{Motivation for investigation}

 There are several motivations for us to investigate the basic stochastic partial differential equations (PDEs) one might wish to solve, either by extending Ito’s theory \cite{Dalang1999} and \cite{peszat1997} or by Malliavin calculus,see \cite{malliavincalc}.
 \begin{itemize}
\item For homogenization problems of PDEs driven by highly oscillating stationary random fields (see Iftimie et al.~\cite{Iftimie2008}). Here we notice that limit theorems are often obtained through a Feynman-Kac representation of the solution to the heat equation, but for the wave equation ,there is no Feynman-Kac representation, so we need another approach.
\item There is a connection between equation \eqref{eqn:DO process} and the partition function of directed and undirected continuum polymers. This link has been exploited in Rovira and Tindel~\cite{tindel2005} and is particularly present in [1], where basic properties of an equation of type \eqref{eqn:DO process} are translated into corresponding properties of the polymer.
\item The multiplicative stochastic heat equation exhibits concentration properties of its energy. This interesting phenomenon is referred to as intermittency for the process $u$ solution to (1.1),see Conus, Joseph, Khoshnevisan~\cite{conuskhoshnevisan2013}, and as a localization property for the polymer measure Carmona and Hu~\cite{carmonahu2006}. The intermittency property for our model is one of the main result of the current paper, and will be developed in Section 1.3.
\item We point out that the stochastic heat equation is related to the Kardar-Parisi-Zhang(KPZ) equation\cite{KPZeqn} by Hopf-Cole transformation:
 \begin{align}
     \frac{\partial h}{\partial t}=\Delta h- |\nabla h|^2+\lambda \dot{W}(t,x),
 \end{align}
 which describes the growth of interfaces such as the clustering of bacteria or the movement of galaxies. The Hopf-Cole transformation is a type of logarithmic transformation that connects the Stochastic heat equation to the KPZ equation. This connection was rigorously proved by Martin Hairer, see \cite{hairer2013}
 \end{itemize}
 For the stochastic wave equation, we have several applications , see \cite{utahsummer2006}. The first example is the motion of a strand of DNA. A DNA molecule can be viewed as a long elastic string. If we describe the position of the string as $u(t,x)$, since a DNA molecule typically “floats” in a fluid, it is constantly in motion. Just as a particle of pollen floating in a fluid moves according to Brownian motion, then by Newton's law of motion, we have
 \begin{align}
      \frac{\partial^2}{\partial t^2} u(t,x)=\Delta u(t,x)+  \int_0^1 k(x,y)u(t,y)\,dy+\dot{F}(t,x),
 \end{align}
where the first term on the right-hand side represents the elastic forces, the second term is a (non-local) friction term, and the third term $\dot{F}(t,y)$ is a Gaussian noise, with spatial correlation $k$, that is,
$E(\dot{F}(t,x)\dot{F}(s,y))=\delta_0(t-s)k(x,y)$
where $\delta_0$ denotes the Dirac delta function. The function $k$ is the same in the friction term and in the correlation.\\
A second example is the internal structure of the sun, an international project named Project SOHO (Solar and Heliospheric Observatory), whose main objective was the motion of the sun’s surface to obtain information about the internal structure of the sun. They used a model given by
\begin{align}
    \frac{\partial^2 u}{\partial t^2} (t,x)=c^2(x)\rho_0(x)\Bigg{(}\nabla \cdot (\frac{1}{\rho_0(x)}\nabla u)+\nabla \cdot F(t,x)\Bigg{)},
\end{align}
where $x\in B(0,R)$, the ball centered at the origin with radius $R$, $c^2(x)$ is the speed of wave propagation at position $x$, $\rho_0(x)$ is the density at position x and the vector $F(t,x)$ models the shock that originates at time $t$ and position $x$.\\
A model for F that corresponds to the description of the situation would be 3-dimensional Gaussian noise concentrated on the sphere $\partial B(0 , r)$, where $0 < r < R$, see \cite{Dalang2004}.



\section{Intermittency}
In this section , we will introduce the notion of Lyapunov exponent, which is widely used in the literature to establish intermittency properties, see \cite[Theorem 2.2]{Foondun2008}, \cite[Chapter 1]{carmona1994}. In the physics literature, a space–time random field is called \emph{physically intermittent} if it develops very high peaks concentrated on small spatial islands, as time becomes large \cite{BertiniCancrini}. To give a formal mathematical definition of intermittency for a random-field $u = \{u(t, x); t \geq 0, x \in \mathbb{R}^d \}$, we consider the upper Lyapunov exponent
\begin{definition}[Lyapunov exponent]
The upper pth moment Lyapunov exponent is defined as \\
\begin{align}
    \gamma(p):=\limsup_{t\rightarrow \infty} \frac{1}{t} \ln \sup_{x\in \mathbb{R}^d}E(|u(t,x_0)|^p) \hspace{8mm} \text{for all } p \in (0,\infty).
\end{align}
\end{definition}
\begin{definition}[Full Intermittency]
Let $p$ be the smallest integer for which  $\gamma(p)>0$. As usual we use the convention that the infimum of the empty set is $\infty$. When
$p<\infty$, we say that the solution field $u(t,x)$ shows (asymptotic) intermittency of order
$p$. A random field $u$ is fully intermittent if $p\mapsto \gamma(p)/p$ is strictly increasing for all $p \geq 2$. The definition is motivated by the convexity of $\gamma(p)$. See Carmona and Molchanov~\cite[Theorem III.1.2]{carmona1994} for details.
\end{definition}
\begin{definition}[Weak Intermittency]
The random field $u$ is called weakly intermittent if, regardless of $x_0$ 
\begin{align}
    \gamma(2)>0 \hspace{4mm}\text{ and } \hspace{4mm}\gamma(p)<\infty \hspace{4mm}\text{ for all }  p\geq 2.
\end{align}
If $\gamma(1)=0$ and $u(t,x)\geq 0$ almost surely, then weak intermittency implies full intermittency.
\end{definition}
Several results have already been established in the literature for intermittency of the solution to SPDEs. Intermittency for the heat equation with white noise has been established in Foondun and Khoshnevisan~\cite{Foondun2008}. Dalang, Mueller~\cite{Mueller2009} studied wave equation driven by white noise.

Also, Conus and Balan~\cite{Balan2016} managed to prove that we can treat the spatial white noise as a special case of fractional noise, and get the intermittency level of the second moment of SHE and SWE solution. Here the main technique was a Feynman-Kac type representation of the moments with Poisson process. We will take advantage of a similar representation in Chapter 4 to established the lower bound on the Lyapunov exponent. Hu et al.~\cite{HuHuangNualartTindel} managed to prove the intermittency for the stochastic heat equation with any order while establishing a Feynman Kac formula. Our generalized fractional noise techniques are mainly inspired by those two papers.


\begin{remark}
We have a few comments regarding the intermittency result.
\begin{itemize}
    \item In the end, we manage to prove that the intermittency level only depends on the order of $t$. Hence, the equation driven by an interpolation of DO noise and fractional Brownian motion will maintain the same intermittency level. See Appendix Remark~\ref{covariancedoesnotmatter}.
    \item In general, the results on intermittency will hold for any initial conditions such that $0\leq u_0\leq C_1$ and (for the wave equation) $|v_0|\leq C_2$, where $C_1,C_2$ are universal constant. For simplicity we will only focus on the case where $u_0$ and $v_0$ are constant.
\end{itemize}

\end{remark} 

The general conjecture that we aim to investigate is that intermittency level is only determined by the variance of the noise but not the specific covariance structure, check the Appendix Remark~\ref{covariancedoesnotmatter}.
 
The dissertation is organized as follows. The second chapter will focus on the existence and uniqueness of the solution to \eqref{eqn:DO process}
and \eqref{eqnwave:DO process}. The third chapter will discuss the derivation of the nth moment formula. The fourth chapter will cover the Lyapunov exponent of our solution (both upper and lower bound of the solution). From Chapter 5 to Chapter 8, we will follow a similar order but with a generalized fractional noise interpolating between the DO noise and the standard fractional noise. Finally some technical results are gathered in the Appendix.


==> paste.tex <==
\begin{theorem} \label{thm:2nd_mom_formula}

Consider a Poisson process $(N_t)_{t \geq 0}$ with rate 1, and let $(\tau_n)_{n \geq 0}$ denote its jump times. Also, consider $B^{(i)} = \left(B^{(i)}_t\right)_{t \geq 0}$ to be i.i.d copies of a standard Brownian motion. We define a stochastic process $X = (X_t)_{t \geq 0}$ as follows: for $0 < t \leq \tau_1$, let
$$X_t = X_0 + B^{(1)}_t.$$
For $i \geq 1$ and $\tau_i < t \leq \tau_{i+1}$, let
$$X_t = X_{\tau_i} + B^{(i+1)}_{t - \tau_i}.$$
We denote by $P_x$ the probability measure under which $X_0 = x$ and $E_x$ the expected value under $P_x$.
We have
\begin{align}
\no \lefteqn{E[u(t,x)u(t,y)] }\\
&= e^t E_x\left[\lambda^2 w(t - \tau_{N_t}, X^{1}_{\tau_{N_t}}) w(t - \tau_{N_t}, X^{2}_{\tau_{N_t}}) \prod_{i=1}^{N_t} \left((t-\tau_i)^{2H-1} f(X^1_{\tau_i} - X^2_{\tau_i})\right)\right],
\end{align}
where $X^1$ and $X^2$ are two i.i.d copies of the process $X$ defined above.

Notice that for the heat equation,
$p_h(t,\mathbb{R}^d)=1$ for all $d\geq 1$.\\
\end{theorem}
Theorem \ref{thm:2nd_mom_formula} extends to higher moments as follows. Let $P_n$ denote the set of unordered pairs from $\mathcal{L}_n= \{1,...,n\}$ 
and for $\rho\in \mathcal{P}_n$, we write $\rho = \{\rho_1,\rho_2\}$, with $\rho_1<\rho_2$. Note that the number of the total pair is equal to  $\nu_n=n(n-1)/2$.
\begin{theorem}
\label{thm:nth moment formula}
The nth moment formula for the heat equation with DO process \\
\begin{align}
\label{initial value heat}
    w(t,x)=u_0
\end{align}
For the wave equation,
\begin{align}
    \label{initial value wave}
    w(t,x)=u_0+t v_0
\end{align}
where $v_0=\frac{\partial u}{\partial t}w(0,x)$
\end{theorem}


For the probabilistic representation, we use the following additional assumption
on the kernel $S(t, dy)$ used in the integral equation \eqref{eqn:solution}.\\
We begin by some settings on our processes.\\
\begin{definition}
There exists a jointly measurable process $(\tilde{X}_t,t>0)$ such that for each $t>0$\\
\begin{align}
    P(-\tilde{X}_t\in dx)=\frac{|S(t,dx)|}{|S(t,\mathbb{R}^d)|}
\end{align}
Notice that if $S(t,A)=S(t,-A)$, the minus sign in front of $\tilde{X}_t$ is not needed.
\end{definition}
There are some typical examples that helps to understand the model.
\begin{enumerate}
    \item The heat equation. In this case ,one can take $\tilde{X}_t=\sqrt{t}X_0$, where $X_0$ is a standard $N(0,\mathcal{I}_d)$ random vector in $\mathbb{R}^d$. An alternative possibility is to let $\tilde{X}_t$ be a standard Brownian motion in $\mathbb{R}^d$\\
    \item The wave equation. In the three dimensional case, one can take $\tilde{X}_t=t\Theta_0$, where $\Theta_0$ is chosen according to the uniform probability measure on $\partial B(0, 1)$. The one and two dimensional cases can be handled in a similar way.
\end{enumerate}
Let $\tilde{X}^{(i)} = (\tilde{X}_t^{(i)}, t \geq 0), i \geq  1$, be i.i.d. copies of $(\tilde{X}_t, t \geq 0)$, and let$ (N(t), t \geq0)$ be a rate one Poisson process independent of the $(\tilde{X}^{(i)})$. Let $0 < \tau_1 < \tau_2<\cdot$
be the jump times of $(N(t))$ and set $\tau_0 \equiv 0$. Deﬁne a process $X = (X_t, t \geq 0)$ as follows:

$X_t = X0 +\tilde{X}_t^{(1)}$ for $0 \leq t \leq \tau_1$,\\

and for $i \geq 1$,\\

$X_t = X_{\tau_i} + \tilde{X}_{t-\tau_i}^{(i+1)}$ , for $\tau_i < t \leq \tau_{i+1}$.\\
We use $P_x$ to denote a probability under which, in addition, $X_0 = x$ with prob-
ability one. Informally, the process $X$ follows $\tilde{X}^{(1)}$ during the interval $[0,\tau_1]$, then
follows $\tilde{X}^{(2)}$ started at $X_{\tau_1}$ during $[\tau_1,\tau_2]$, then $\tilde{X}^{(3)}$ started at $X_{\tau_2}$ during $[\tau_2,\tau_3]$,
etc. See Figure 1 for an illustration.



\begin{proof*}
By a standard argument for non-linear SPDE of affine type (e.g. Parabolic Anderson model, see \cite{carmona1994}), it is easy to see that the process $u(t,x)$ can be written as 
$$u(t,x) = \sum_{m=0}^{\infty} I_m(t,x),$$
where $I_0(t,x) = w(t,x)$ and, for $m \geq 1$, the process is defined inductively by 
$$I_m(t,x) =  \int_{0}^{t} \int_{\R^d} s^{H-1/2} p_{t-s}(x-z) I_{m-1}(s,z) W(ds,dz).$$
Note that the $I_m$ are orthogonal in $L^2(\Omega)$, since they are all in Wiener chaoses of different order.

We will prove by induction on $m$ that
\begin{equation} \label{eqn:2nd_mom_Im}
E[I_m(t,x)I_m(t,y)] = J_m(t,x,y),
\end{equation}
where
\begin{align*} 
J_m(t,x,y) = E_x\left[\ind_{\{N_t = m\}} w(t - \tau_m, X^{1}_{\tau_m}) w(t - \tau_m, X^{2}_{\tau_m}) \prod_{i=1}^{m} \left((t-\tau_i)^{2H-1} f\left(X^1_{\tau_i} - X^2_{\tau_i}\right)\right) \right].
\end{align*}
Once this is established, the result of Theorem \ref{thm:2nd_mom_formula} follows by direct summation on $m$ using the orthogonality of the processes $I_m$.

Equation \eqref{eqn:2nd_mom_Im} in the case $m=0$ is immediate. We now assume that \eqref{eqn:2nd_mom_Im} holds up to $m-1$ and will establish the result for $m$. Let $\mathcal{F}_1 = \sigma(\tau_1, X^1_{\tau_1}, X^2_{\tau_1})$. By standard results on conditional expectations, we can write
\begin{align*}
\lefteqn{J_m(t,x,y)} \\
& = E_x\left[\ind_{\{\tau_1 \leq t\}} e^{\tau_1} (t-\tau_1)^{2H-1} f\left(X^1_{\tau_1} - X^2_{\tau_1}\right) \phantom{\prod_{i=2}^{m}} \right. \\
& \qquad \left. E_x\left[\ind_{\{N_t-N_{\tau_1} = m-1\}} w(t - \tau_m, X^{1}_{\tau_m}) w(t - \tau_m, X^{2}_{\tau_m}) \prod_{i=2}^{m} \left((t-\tau_i)^{2H-1} f\left(X^1_{\tau_i} - X^2_{\tau_i}\right)\right) \mid \mathcal{F}_1 \right] \right].
\end{align*}
By the strong Markov property of the Poisson process $(N_t)$ at time $\tau_1$, the independence and stationarity of the increments of the processes $X^{i}$ ($i=1,2$) up to and after $\tau_1$, the conditional expectation above is equal to $J_{m-1}(t-\tau_1,X^1_{\tau_1},X^2_{\tau_2})$. Hence, we obtain
\begin{align*}
J_m(t,x,y) & = E_x\left[\ind_{\{\tau_1 \leq t\}} e^{\tau_1} (t-\tau_1)^{2H-1} f\left(X^1_{\tau_1} - X^2_{\tau_1}\right) J_{m-1}(t-\tau_1,X^1_{\tau_1},X^2_{\tau_1}) \right].
\end{align*}
Using first the fact that the random variables $X^{1}_t$ and $X^{2}_t$ are independent, both with centered normal distribution with variance $t$, and then that the law of $\tau_1$ is exponential with parameter 1, we can rewrite the expectation as an integral. Namely,
\begin{align*}
\lefteqn{J_m(t,x,y)} \\
 & = E\left[ \ind_{\{\tau_1 \leq t\}} e^{\tau_1} (t-\tau_1)^{2H-1} \phantom{\int_{\R}} \right. \\
 & \qquad \times \left. \int_{\R} dz_1 \int_{\R} dz_2 \, p_{\tau_1}(x-z_1) p_{\tau_1}(x-z_2) f\left(z_1 - z_2\right) J_{m-1}(t-\tau_1,z_1,z_2) \right] \\
 & = \int_{0}^{\infty} ds \, e^{-s} \ind_{\{s \leq t\}} e^{s} (t-s)^{2H-1} \\
 & \qquad \times \int_{\R} dz_1 \int_{\R} dz_2 \, p_{s}(x-z_1) p_{s}(y-z_2) f\left(z_1 - z_2\right) J_{m-1}(t-s,z_1,z_2) \\
  & = \int_{0}^{t} ds \, s^{2H-1} \int_{\R} dz_1 \int_{\R} dz_2 \, p_{t-s}(x-z_1) p_{t-s}(y-z_2) f\left(z_1 - z_2\right) J_{m-1}(s,z_1,z_2).
\end{align*}
Now, using the induction assumption, we can write $J_{m-1}$ as an expectation in the terms of the process $I_m$. Using standard results about moments of Walsh integrals, we obtain
\begin{align*}
\lefteqn{J_m(t,x,y)} \\
& = \int_{0}^{t} ds \, s^{2H-1} \int_{\R} dz_1 \int_{\R} dz_2 \, p_{t-s}(x-z_1) p_{t-s}(y-z_2) f\left(z_1 - z_2\right) E[I_{m-1}(s,z_1)I_{m-1}(s,z_2)] \\
& = E\left[\int_{0}^{t} \int_{\R} s^{H-1/2} p_{t-s}(x-z_1) I_{m-1}(s,z_1) W(ds,dz_1) \right. \\
& \qquad \qquad \times \left. \int_{0}^{t} \int_{\R} s^{H-1/2} p_{t-s}(y-z_2) I_{m-1}(s,z_2) W(ds,dz_2) \right] \\
& = E[I_m(t,x)I_m(t,y)].
\end{align*}
The result is proved.
\end{proof*}

